Ellipsotopes: Combining Ellipsoids and Zonotopes for Reachability Analysis and Fault Detection

Ellipsoids are a common representation for reachability analysis, because they can be transformed efficiently under affine maps, and allow conservative approximation of Minkowski sums, which let one incorporate uncertainty and linearization error in a dynamical system by expanding the size of the reachable set. Zonotopes, a type of symmetric, convex polytope, are similarly frequently used due to efficient numerical implementation of affine maps and exact Minkowski sums. Both of these representations also enable efficient, convex collision detection for fault detection or formal verification tasks, wherein one checks if the reachable set of a system collides (i.e., intersects) with an unsafe set. However, both representations often result in conservative representations for reachable sets of arbitrary systems, and neither is closed under intersection. Recently, representations such as constrained zonotopes and constrained polynomial zonotopes have been shown to overcome some of these conservativeness challenges, and are closed under intersection. However, constrained zonotopes can not represent shapes with smooth boundaries such as ellipsoids, and constrained polynomial zonotopes can require solving a non-convex program for collision checking or fault detection. This paper introduces ellipsotopes, a set representation that is closed under affine maps, Minkowski sums, and intersections. Ellipsotopes combine the advantages of ellipsoids and zonotopes while ensuring convex collision checking. The utility of this representation is demonstrated on several examples.

==> sections/00_outline.tex <==
\section*{Outline}
\begin{outline}[enumerate]
    \1 Geometric set representations for robotics
        \2 Sets as basic computational objects
        \2 Reachable or invariant sets of dynamical systems
        \2 Sets of states or parameters consistent with a bounded-error model
        \2 Importance of set operations/transformations
        \2 Importance of collision checking
    \1 Types of set representations
        \2 Convex sets
            \3 Intervals
            \3 Polytopes
            \3 Signed distance collision checking for convex sets
                \4 \cite{zhang2018optimizationbased_collision_avoidance} \cite{lutz2021efficient_optimization_based_collision_avoidance}
                \4 These signed distance things also require solving optimization programs
            \3 Zonotopes
                \4 Constrained zonotopes \cite{scott2016constrained_zonotopes}
                \4 \textbf{Weaknesses:} can't represent "smooth" objects
            \3 Ellipses and Ellipsoids
                \4 \cite{kurzhanski2000ellipsoidal} \cite{kurzhanskiy2006ellipsoidal_toolbox}
                \4 \textbf{Advantages:} analytic way to check if a point is inside them, ``natural'' representation of Gaussian confidence level sets
                \4 \textbf{Disadvantages:} not closed under intersection/convex hull, can't represent "rigid" objects
            \3 Support functions
                \4 \cite{le2010reachability_support_funcs}
                \4 Support functions of convex sets
                \4 \textbf{Strengths:} Linear map, minkowski sum, convex hull
                \4 \textbf{Weaknesses:} No intersection/collision checking?
                Point containment
            \3 Elliptopes
                \4 Convex Euclidean body formed from elements that are vectorized matrices
                \4 Intersection of positive semidefinite cone with set of hyperplanes defined unity main diagonal
            \3 Zonoids
                \4 Limits of zonotopes in the Hausdorff metric
                \4 Limit as you add infinite generators - create smooth objects
                \4 Not practical 
        \2 Non-convex sets
            \3 Star sets
                \4 Logical predicates used to constrain zonotope factors
                
            \3 Level sets
                \4 Can represent any shape using nonlinear functions
            \3 Taylor models
                \4 Consist of a polynomial and interval remainder part
                \4 Generalization: polynomial zonotopes
            \3 Constructive solid geometry (CSG) 
                \4 Implicit point membership classification function
                \4 \cite{lutz2021efficient_optimization_based_collision_avoidance}
                \4 Intersection and union (smooth approximations)
                \4 \textbf{Disadvantage:} Probably hard to do reachability (propagate through dynamical system, linear mapping, minkowski sum, etc.)
            \3 Constrained Polynomial Zonotopes \cite{kochdumper2020cons_poly_zono}
                \4 \textbf{Strengths:} Closed under linear map, Minkowski sum, Cartesian product, convex hull, intersection, union, quadratic and higher order maps. Highly expressive
                \4 \textbf{Disadvantages:} Collision checking is not convex
            \3 Polynotopes \cite{combastel2020polynotopes}
                \4 \textbf{Strengths:} even more flexible than CPZs
                \4 \textbf{Weaknesses:} even worse for collision checking and point containment than CPZs (requires solving mixed-boolean nonconvex programs)
        
    \1 Ellipsotopes: novelty
        \2 Generalize both ellipses and zonotopes
            \3 Can add Gaussian confidence level set directly to a zonotope without needing a p-zonotope
            \3 Enables exact Minkowski sum for ellipsoids, allowing us to represent things like a Gaussian distribution with uncertain mean
        \2 Convex collision checking
            \3 In comparison, (blank) does not have convex collision checking
        \2 In general, adds expressivity and flexibility (to existing set representations), while (mostly) preserving availability and complexity of operations
\end{outline}

==> sections/07_bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/shrey_bio_pic.jpg}}]{Shreyas Kousik}
(Member, IEEE) received the B.S. degree in mechanical engineering from the Georgia Institute of Technology, Atlanta, GA, USA in 2014, and the M.S. and Ph.D. degrees in mechanical engineering from the University of Michigan, Ann Arbor, MI, USA in 2020.
He is currently a postdoctoral scholar at Stanford University, Stanford, CA, USA.
His research focuses on verifiable perception, planning, and control for mobile robots.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/adam_dai_bio_pic.png}}]{Adam Dai}
received the B.S. degree in electrical engineering from the California Institute of Technology, Pasadena, CA, USA in 2019.
He is currently a Ph.D. candidate in the Department of Electrical Engineering at Stanford University.
His research interests include formal guarantees on perception, planning, and control under uncertainty for mobile robots.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/grace_gao_portrait_2019_2.png}}]{Grace Xingxin Gao}
(Senior Member, IEEE)
received the B.S. degree in mechanical engineering and M.S. degree in electronics engineering from Tsinghua University, Beijing, China, in 2001 and 2003, respectively, and received the Ph.D. degree in electrical engineering from Stanford University in 2008. 
She is currently an assistant professor in the Department of Aeronautics and Astronautics at Stanford University.
Her research is on robust and secure positioning, navigation, and timing with applications to manned and unmanned aerial vehicles, robotics and power systems.
\end{IEEEbiography}
